Mastering the ABCDs of Complex Questions: Answer-Based Claim Decomposition for Fine-grained Self-Evaluation

When answering complex questions, large language models (LLMs) may produce answers that do not satisfy all criteria of the question. While existing self-evaluation techniques aim to detect if such answers are correct, these techniques are unable to determine which criteria of the question are satisfied by the generated answers. To address this issue, we propose answer-based claim decomposition (ABCD), a prompting strategy that decomposes questions into a series of true/false claims that can be used to verify which criteria of the input question an answer satisfies. Using the decomposed ABCD claims, we perform fine-grained self-evaluation. Through preliminary experiments on three datasets, including a newly-collected challenge dataset ObscureQA, we find that GPT-3.5 has some ability to determine to what extent its answer satisfies the criteria of the input question, and can give insights into the errors and knowledge gaps of the model.

==> data/ccg.tex <==
\begin{table*}[]
\small
\centering
\setlength{\tabcolsep}{4Pt}
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{3}{c|}{\textbf{Zero-Shot QA}} & \multicolumn{3}{c|}{\textbf{Zero-Shot CCG}} & \multicolumn{3}{c}{\textbf{Self-Consistency}} \\
\multicolumn{1}{c|}{} & $\mathbb{P}$(IDK) & $\mathbb{P}$(I) & $\mathbb{P}$(C) & $\mathbb{P}$(IDK) & $\mathbb{P}$(I) & $\mathbb{P}$(C) & \multicolumn{1}{l}{$\mathbb{P}$(Cons)} & $\mathbb{P}$(C | Cons) & $\mathbb{P}$(Both I | Incons) \\ \midrule
TriviaQA & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
HotpotQA (Easy) & 0.093 & 0.420 & 0.487 & 0.007 & 0.547 & 0.447 & 0.487 & 0.726* & 0.558 \\
HotpotQA (Medium) & 0.213 & 0.393 & 0.393 & 0.007 & 0.667 & 0.327 & 0.340 & 0.745* & 0.677* \\
ObscureQA & 0.050 & 0.695 & 0.255 & 0.000 & 0.810 & 0.190 & 0.330 & 0.455 & 0.784* \\ \bottomrule
\end{tabular}
\vspace{-1.5ex}
\caption{\label{table:ccg}Comparison of question answering (QA) and constrained claim generation (CCG) when applied to GPT 3.5 on our four datasets. $\mathbb{P}$(IDK), $\mathbb{P}$(I), and $\mathbb{P}$(C) are the proportions of answers annotated as non-responses, incorrect, and correct, respectively. $\mathbb{P}$(Cons) is the proportion of answers that were consistent between QA and CCG. $\mathbb{P}$(C | Cons) is the proportion of answers that were correct, given they were consistent. $\mathbb{P}$(Both I | Incons) is the proportion of answers that were both incorrect, given that they were inconsistent.}
\vspace{-2.5ex}
\end{table*}
